See it, Think it, Sorted: Large Multimodal Models are Few-shot Time Series Anomaly Analyzers

Time series anomaly detection (TSAD) is becoming increasingly vital due to the rapid growth of time series data across various sectors. Anomalies in web service data, for example, can signal critical incidents such as system failures or server malfunctions, necessitating timely detection and response. However, most existing TSAD methodologies rely heavily on manual feature engineering or require extensive labeled training data, while also offering limited interpretability. To address these challenges, we introduce a pioneering framework called the Time Series Anomaly Multimodal Analyzer (TAMA), which leverages the power of Large Multimodal Models (LMMs) to enhance both the detection and interpretation of anomalies in time series data. By converting time series into visual formats that LMMs can efficiently process, TAMA leverages few-shot in-context learning capabilities to reduce dependence on extensive labeled datasets. Our methodology is validated through rigorous experimentation on multiple real-world datasets, where TAMA consistently outperforms state-of-the-art methods in TSAD tasks. Additionally, TAMA provides rich, natural language-based semantic analysis, offering deeper insights into the nature of detected anomalies. Furthermore, we contribute one of the first open-source datasets that includes anomaly detection labels, anomaly type labels, and contextual description, facilitating broader exploration and advancement within this critical field. Ultimately, TAMA not only excels in anomaly detection but also provides a comprehensive approach for understanding the underlying causes of anomalies, pushing TSAD forward through innovative methodologies and insights.

==> tables/ablation-auxline.tex <==
% \begin{table}[thbp]
% \vspace{-5pt}
% \caption{Mean \emph{AUC-PR} results without point-adjustment. TAMA-R represents the performance using rotated image. Values are multiplied by 100.}
% \label{tab:ablation-auxline}
%     \vspace{-5pt}
%     % \vskip 0.05in
%     % \setlength{\tabcolsep}{2pt}
%     \centering
%     % \begin{small}
%     \resizebox{0.7\columnwidth}{!}{
%     \begin{tabular}{c|c|c}
%       \toprule
%       % Dataset & \multicolumn{2}{c|}{\textbf{NASA-SMAP}}& \multicolumn{2}{c}{\textbf{NASA-MSL}}\\
%       Datasets  & TAMA& TAMA-R\\
%       \midrule
%         UCR   & 77.3 & 32.9~(\textbf{-44.4})\\
%         NASA-SMAP    & 58.6 & 28.6~(\textbf{-30.0})\\
%         % SIGLLM(Text)~\cite{alnegheimish_large_2024}   & 42.9 & 43.1\\
%       \bottomrule
%     \end{tabular}}
% % \end{small}
% \vspace{-10pt}
% \end{table}

==> tables/f1_table.tex <==
\begin{table*}[t!]
    \caption{Quantitative results across six datasets use metrics point-adjusted \emph{F1}, \emph{AUC-PR}, and \emph{AUC-ROC}. Best and second-best results are in bold and underlined, respectively. \textbf{TAMA} represents our framework, and \textbf{TAMA*} represents our framework without self-reflection. In both \textbf{TAMA} and \textbf{TAMA*}, we provide \underline{three} normal references. (Some datasets include more than one series. To present the true performance of each method as much as possible, each unit in the table contains two values: \emph{maxima} / \emph{mean}. The \emph{maxima} represents the best result among all sub-sequences, while the \emph{mean} denotes the average of all sub-sequences. All values are multiplied by 100).}
    \label{tab:main_results}
    \vspace{-5pt}
    % \vskip 1005in
    \centering
    \resizebox{0.9\textwidth}{!}{
    % \begin{small}
    \renewcommand{\multirowsetup}{\centering}
    % \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c|cc|ccc|ccc}
    % UCR, NASA-SMAP, NASA-MSL
    \toprule
    Dataset & \multicolumn{2}{c|}{\textbf{UCR}} & \multicolumn{3}{c|}{\textbf{NASA-SMAP}}& \multicolumn{3}{c}{\textbf{NASA-MSL}}\\
    Category& Point& Shapelet&  Point&  Shapelet& Trend& Shapelet& Seasonal& Trend\\
    \midrule
    % Baseline
    IF          & 77.3 / 24.7& 44.6  /  37.7& 25.3 / 24.4& 94.2 / 54.2& 77.1 / 58.9& 87.7 / 65.0& 88.6 / 47.6& \underline{80.4} / 53.6 88.7 / 68.7 \\
    LOF         & \textbf{100} / 42.8& 50.0 / 35.6& \textbf{99.9} / 92.8& \textbf{100} / 62.2& 61.4 / 43.4& \underline{99.9} / 60.1& 66.8 / 36.4 66.0 / 44.5& 99.8 / 58.6 \\
    TranAD      & 93.7 / 38.2& 51.0 / 30 \textbf{99.9} / 77.0& 99.6 / 59.0& 73.9 / 36.8& \textbf{100} / 74.4& 99.1 / 64.6& 79.6 / 49.2& \underline{99.9} / 82.5  \\
    GDN         & 80.6 / 71.4& 59.0 / 33.4 \textbf{99.9} / 87.1& \textbf{100} / 76.4& 66.2 / 40.8& \textbf{100} / 86.1& \textbf{100} / 85.1& 56.7 / 38.7& \textbf{100} / 93.8 \\
    MAD\_GAN    & 85.0 / \underline{74.2} \underline{65.9} / \underline{51.5}& \textbf{99.9} / \underline{99.4}& \textbf{100} / 61.3& 72.3 / 39.9& \textbf{100} / 83.3& \textbf{100} / {96.0}& 50.0 / 46.4& \textbf{100} / 95.7 \\
    MSCRED      & 96.0 / 32.6& 45.9 / 28.9 \textbf{99.9} / 94.2& \underline{97.9} / 57.0& 61.7 / 40.8& \textbf{100} / 77.0& 92.2 / 63.0& 51.8 / 39.5& 98.1 / 73.2 \\
    MTAD\_GAT    & 36.6 / 14.8& 38.9 / 34.2 \underline{94.4} / 84.6& \textbf{100} / 78.3& 58.0 / 40.2& \textbf{100} / 77.0& \textbf{100} / 90.6& 67.8 / 49.2& \textbf{100} / 81.2 \\
    OminiAnomaly& 95.7 / 34.5& 45.9 / 26.0 \textbf{99.9} / 85.6& \textbf{100} / 57.1& 63.2 / 43.6& \textbf{100} / 77.5& \textbf{100} / 71.4 74.9 / 40.0& \underline{99.9} / 85.0 \\
    USAD        & \textbf{100} / 57.6 50.0 / 33.1& \textbf{99.9} / 97.1& \textbf{100} / 72.8& 63.2 / 43.6& \textbf{100} / 93.9& \underline{99.9} / 91.6& 60.8 / 42.6& \textbf{100} / \underline{94.2} \\
    SIGLLM (GPT-4o) & 44.6 / 23.1& 15.5 / 7.4 96.5 / 93.5& 97.8 / 69.0& 49.2 / 29.1& 99.8 / 95.5& 97.9 / 70.7& 100.0 / 72.4& 100.0 / 90.0 \\
    \midrule
    % Our approaches
    \textbf{TAMA}  & \underline{97.6} / \textbf{92.5}& \textbf{97.7} / \textbf{93.0}& \textbf{99.9} / \textbf{99.8}& \textbf{100} / \textbf{94.5} \textbf{100} / \textbf{95.5}& \textbf{100} / \textbf{98.4}& \textbf{100} / \textbf{97.}5& \textbf{100} / \textbf{99.4}& \textbf{100} / \textbf{99.8} \\
    \textbf{TAMA*} & \underline{97.6} / \textbf{92.5}& \textbf{97.7} / \textbf{93.0}& \textbf{99.9} / \textbf{99.8}& \textbf{100} / \underline{87.8}& \textbf{100} / \underline{89.2}& \textbf{100} / \underline{97.0}& \textbf{100} / \underline{96.1} \textbf{100} / \underline{97.7}& \textbf{100} / \underline{99.0} \\
    \midrule
    % NormA, ECG, Dodgers
    \midrule
    % Dataset & \multicolumn{3}{c|}{\textbf{SMD}} & \multicolumn{3}{c|}{\textbf{ECG}} & \multicolumn{3}{c}{\textbf{Dodgers}}\\
    % Metric& F1& AUC-PR& AUC-ROC& F1& AUC-PR& AUC-ROC& F1& AUC-PR& AUC-ROC\\
    % \midrule
    % IF          & \textbf{100} / \textbf{83.9}& 97.0 / 73.8& \textbf{100} / \underline{99.5}& 99.0 / \underline{80.8}& 92.2 / 73.4& \textbf{100} / \textbf{97.2}& 48.4 / 48.4& 52.2 / 52.2& \textbf{89.4} / \textbf{89.4}  \\
    % LOF         & 75.2 / 27.8& 64.6 / 39.9& 59.3 / 52.9& 39.8 / 21.8& 60.7 / 41.4& 84.2 / 56.3& 45.3 / 45.3& 40.8 / 40.8& 63.0 / 63.0 \\
    % TranAD      & 99.6 / 77.0& 91.0 / 70.9& \textbf{100} / 96.8& 98.9 / 69.1& 97.7 / 74.7& \textbf{100} / 94.9& 38.2 / 38.2& 33.9 / 33.9& 74.6 / 74.6  \\
    % GDN         & 99.7 / 76.9& 88.6 / 55.0& \textbf{100} / 77.0& 96.2 / 75.2& 97.4 / 76.6& \underline{99.9} / \underline{96.9}& 37.0 / 37.0& 31.3 / 31.3& 74.2 / 74.2 \\
    % MAD\_GAN    & 92.6 / 67.1& 87.5 / 61.7& \textbf{100} / 91.7& \underline{99.3} / 79.1& 97.6 / 79.2& \textbf{100} / \underline{96.9}& 32.2 / 32.2& 28.6 / 28.6& 74.7 / 74.7 \\
    % MSCRED      & 95.7 / 69.4& 96.2 / 55.8& \textbf{100} / 95.0& 99.0 / 66.4& 97.2 / 73.8& \textbf{100} / 88.7& 37.8 / 37.8& 30.6 / 30.6& 74.6 / 74.6 \\
    % MTAD\_GAT   & 95.3 / 69.7& 90.4 / 59.5& \underline{99.7} / 90.6& \textbf{100} / 67.5& \textbf{98.8} / 73.5& \textbf{100} / 82.5& 39.1 / 39.1& 36.0 / 36.0& 74.9 / 74.9 \\
    % OmniAnomaly& 96.4 / 66.0& 91.8 / 61.6& \textbf{100} / 87.7& 98.6 / 76.8& 97.5 / 76.4& \textbf{100} / 93.5& 33.6 / 33.6& 35.4 / 35.4& 60.3 / 60.3 \\
    % USAD        & \underline{99.7} / 72.2& 93.5 / 67.8& \textbf{100} / 94.4& 96.9 / 71.5& \underline{98.3} / 75.2& \textbf{100} / 94.9& 37.8 / 37.8& 33.1 / 33.1& 74.6 / 74.6 \\
    % SIGLLM (GPT-4o) & 59.8 / 42.9& 53.1 / 30.4& 77.8 / 68.8& 50.4 / 19.2& 87.6 / 71.0& 96.9 / 94.2& 48.1 / 48.1& 60.7 / 60.7& 83.2 / 83.2 \\
    % \midrule
    % \textbf{TAMA}  & \textbf{100} / \underline{77.8}& \textbf{100} / \textbf{87.9}& \textbf{100} / 98.9& 87.5 / \textbf{81.3}& 90.0 / \textbf{84.5}& 99.4 / 95.4& \underline{64.5} / \underline{64.5}& \underline{73.6} / \underline{73.6}& \underline{85.3} / \underline{85.3} \\
    % \textbf{TAMA*} & 93.0 / 62.8& \underline{97.2} / \underline{78.6}& \underline{99.7} / \textbf{99.7} & 88.0 / 78.1& 91.1 / \underline{83.4}& 99.1 / 94.7& \textbf{65.6} / \textbf{65.6}& \textbf{74.0} / \textbf{74.0}& 85.2 / 85.2 \\
    \bottomrule
    \end{tabular}
    % \end{small}
    }
    % \vspace{-10pt}
\end{table*}
